Sound Borrow-Checking for Rust via Symbolic Semantics (Long Version)

The Rust programming language continues to rise in popularity, and as such, warrants the close attention of the programming languages community. In this work, we present a new foundational contribution towards the theoretical understanding of Rust's semantics. We prove that LLBC, a high-level, borrow-centric model previously proposed for Rust's semantics and execution, is sound with regards to a low-level pointer-based language \`a la CompCert. Specifically, we prove the following: that LLBC is a correct view over a traditional model of execution; that LLBC's symbolic semantics are a correct abstraction of LLBC programs; and that LLBC's symbolic semantics act as a borrow-checker for LLBC, i.e. that symbolically-checked LLBC programs do not get stuck when executed on a heap-and-addresses model of execution. To prove these results, we introduce a new proof style that considerably simplifies our proofs of simulation, which relies on a notion of hybrid states. Equipped with this reasoning framework, we show that a new addition to LLBC's symbolic semantics, namely a join operation, preserves the abstraction and borrow-checking properties. This in turn allows us to add support for loops to the Aeneas framework; we show, using a series of examples and case studies, that this unlocks new expressive power for Aeneas.

==> Makefile <==
.PHONY: all clean

all:
	latexmk -pdf -pvc -shell-escape paper.tex

clean:
	latexmk -c
	rm -rf *.aux *.bbl *.blg *.fls *.log *.fdb_latexmk *.out *.synctex.gz *.pyg

# To submit online
.PHONY: online
online:
	mkdir -p online
	cp acmart.cls online/
	cp ACM-Reference-Format.bst online/
	cp paper.bbl online/
	cp paper.bib online/
	cp paper.tex online/
	cp -r _minted-paper online/
	cp Makefile online/
	cp LlbcSimulationsDiagram.png online/
	sed -i 's/%\\usepackage\[frozencache=true\]{minted}/\\usepackage\[frozencache=true\]{minted}/' online/paper.tex
	sed -i 's/\\usepackage\[frozencache=false,finalizecache=true\]{minted}//' online/paper.tex
	rm online.zip && zip -r online online

